Adversarial Robustness on In- and Out-Distribution Improves Explainability

Neural networks have led to major improvements in image classification but suffer from being non-robust to adversarial changes, unreliable uncertainty estimates on out-distribution samples and their inscrutable black-box decisions. In this work we propose RATIO, a training procedure for Robustness via Adversarial Training on In- and Out-distribution, which leads to robust models with reliable and robust confidence estimates on the out-distribution. RATIO has similar generative properties to adversarial training so that visual counterfactuals produce class specific features. While adversarial training comes at the price of lower clean accuracy, RATIO achieves state-of-the-art $l_2$-adversarial robustness on CIFAR10 and maintains better clean accuracy.

==> figs/counter_cifar.tex <==
\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
\newlength{\breite}
\breite1.5cm

\begin{figure}[t!]
\begin{tabular}{p{1cm}x{\breite}x{\breite}x{\breite}x{\breite}x{\breite}x{\breite}x{\breite}x{\breite}}
Model  & Orig. & $\epsilon=0.5$ & $\epsilon=1.0$ & $\epsilon=1.5$ & $\epsilon=2.0$ & $\epsilon=2.5$ & $\epsilon=3.0$\\
\begin{turn}{90} \hspace{-.4cm} Plain \end{turn} & \multicolumn{7}{c}{\includegraphics[width=0.91\textwidth,valign=c]{pics/test_cifar10.pdf}} \\
%\includegraphics[width=0.91\textwidth,valign=c]{pics/test_cifar10.pdf}
\end{tabular}
\caption{\label{fig:plain-cf} Attempt at visual counterfactuals for a plain model. The targeted attack immediately produces very high confidence in the class
but instead of class features only high-frequency noise appears because plain models are not robust.}
\end{figure}

A \textit{visual counterfactual explanation} of our classifier $f$ for a given budget $\epsilon$, original point $x$ and target class $t \in \{1,\ldots,K\}$ is defined as
\begin{equation}\label{eq:vf} x^{(t)} = \argmax_{z \in [0,1]^d, \norm{x-z}_2 \leq \epsilon} \hat{p}_{f,t}(z),
\end{equation}
where $\hat{p}_{f,t}(z)$ is the confidence for class $t$ of our classifier for the image $z$. The optimization to get a visual counterfactual is essentially identical to a targeted attack with an $l_2$-threat model of budget $\epsilon$. This method can only produce meaningful counterfactuals if the confidence of the classifier is a reliable quantity in the whole image space
(or at least the ranking of the images via the confidence is aligned with the ranking of emerging features). 


==> res/cifar10_id_revised.tex <==
\newcommand{\svhnIDr}{11.81mm}

\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\definecolor{rred}{rgb}{.0,0.0,0.0}
\begin{table}[t]
\begin{center}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.0}
\caption{\label{Tab:IDRobustness_cifar10_revised} \textit{ID performance:} Corrected robust test accuracy of Table \ref{Tab:IDRobustness_cifar10}	for different threat models after fixing a small bug in AutoAttack \cite{CroHei2020} which lead to an \textit{underestimation} of the robust test accuracy.
% Values that differ from Table \ref{Tab:IDRobustness_cifar10_revised} by more than $0.05\%$ are marked in red.
}
\begin{tabular}{p{\firstcolumnID}|ccccccccc}
\hline
CIFAR10 & Plain &  OE  & ACET  & M$_{0.5}$ &  AT$_{0.5}$ & AT$_{0.25}$ & JEM-0 &  R$_{0.5}$ & R$_{0.25}$ \\
\hline
Clean                   & 96.15   & \textbf{96.41} & 94.06 & 90.83 & 90.79 & 94.00 & 92.84 &  91.08           & 93.53   \\
$l_2$ $0.5$             &  0.00   & 0.01          & {\color{rred}52.66} & 69.32 &               70.42 & 65.02               & {\color{rred}40.67} &  \textbf{73.27}  &  {\color{rred}70.49}  \\
$l_2$ $1.0$             &  0.00   & 0.00          & {\color{rred}14.95} & 36.86 & {\color{rred}38.20} & 20.83               & 6.77 &  \textbf{44.09}  &  {\color{rred}34.15}  \\
$l_{\infty}$ $8/255$    &  0.00   & 0.00          & {\color{rred}12.66} & 29.59 & {\color{rred}30.58} & {\color{rred}14.30} & 7.19 &  {\color{rred}\textbf{37.71}}  &  {\color{rred}29.18}  \\
\hline
\end{tabular}

%\setlength{\tabcolsep}{8.18pt}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{p{\firstcolumnID}|C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}C{\svhnIDr}}
\hline
SVHN & Plain & OE & ACET & AT$_{0.5}$ & AT$_{0.25}$ &  R$_{0.5}$ & R$_{0.25}$ \\
\hline
Clean                &  97.33 & 97.56 & \textbf{97.77} &  94.38 & 96.70 & 94.30          & 96.80  \\
$l_2$ $0.5$          &   0.85 &  0.33 &          28.82 & 68.58 & 63.18 &\textbf{68.85} & 65.02  \\
$l_2$ $1.0$          &   0.01 &  0.00 &           4.20 & 26.40 & 17.19 & \textbf{27.06} & 20.30  \\
$l_{\infty}$ $8/255$ &   0.00 &  0.00 &           4.03 &  27.56 & 19.05 & \textbf{28.20} & 22.14  \\
\hline
\end{tabular}
\end{center}
\vspace{-.6cm}
\end{table}




==> res/cifar10_ood_backup.tex <==
\begin{table}
\begin{center}
\setlength{\tabcolsep}{4.3pt}
\renewcommand{\arraystretch}{1.0}
\caption{\label{Tab:OOD} \textit{OOD performance:} The area under the ROC curve (AUC) on the binary detection task of separating the in- from the out-distribution based on the confidence. The first table shows the average-case performance and worst-case AUC with a threat model $l_2=1.0$ around the out-distribution samples.}
\begin{tabular}{l|cccccccccc}
\hline
Av. Case & Plain &  OE & EBM & Acet & M$_{0.5}$ & M$_{0.25}$ & AT$_{0.5}$ & AT$_{0.25}$ &  R$_{0.5}$ & R$_{0.25}$ \\
\hline
SVHN         &  96.8 & & 89.3 &  95.0  &  91.9 &  93.3 &  93.5 &   95.3 &  96.5 &   96.4 \\
CIFAR100     &  91.6 &  & 87.6 &  89.9  &  84.3 &  87.7 &  85.3 &   89.1 &  90.8 &   91.6 \\
LSUN\_CR      &  95.6 & &  91.6 &  97.8  &  89.7 &  91.3 &  90.7 &   92.5 &  98.0 &   98.3 \\
Imagenet-    &  91.6 &  & 86.7 &  91.5  &  84.8 &  87.6 &  85.9 &   89.0 &  90.5 &   91.3 \\
Noise        &  94.3 &  & 83.1 &  96.5  &  93.7 &  92.4 &  94.9 &   95.5 &  97.8 &   97.6 \\
Uni. Noise &  95.0 &  & 11.8 &  77.3  &  46.1 &  84.4 &  83.2 &   94.6 &  99.9 &   99.9 \\
\hline
\hline
W. Case & Plain & OE & EBM & Acet & M$_{0.5}$ & M$_{0.25}$ & AT$_{0.5}$ & AT$_{0.25}$ &  R$_{0.5}$ & R$_{0.25}$ \\
\hline
SVHN         &   0.0 &  &  & (18.2) & 57.1 &   &  62.0 &   40.1 &   \textbf{81.3} &   81.1 \\
CIFAR100     &   0.0 &  &  & ( 6.0) & 47.9 &   &  48.5 &   31.8 &   71.9 &   \textbf{73.0} \\
LSUN\_CR     &   0.0 &  &  & ( 8.6) & 52.0 &   &  52.8 &   36.5 &   87.3 &   \textbf{89.1} \\
Imagenet-    &   0.0 &  &  & ( 7.4) & 50.6 &   &  51.1 &   36.8 &   72.4 &   \textbf{73.5} \\
Noise        &   0.0 &  &  & (30.4) & 62.5 &   &  68.8 &   39.8 &   88.7 &   \textbf{88.9} \\
Uni. Noise   &       &  &  & (15.0) & 20.7 &   &  62.0 &   67.8 &   \textbf{99.8} &   \textbf{99.8} \\
\hline
\end{tabular}
\end{center}
\end{table}


==> res/svhn_ood.tex <==


